Estimating the Impact of Weather on Agriculture

This paper quantifies the significance and magnitude of the effect of measurement error in remote sensing weather data in the analysis of smallholder agricultural productivity. The analysis leverages 17 rounds of nationally-representative, panel household survey data from six countries in Sub-Saharan Africa. These data are spatially-linked with a range of geospatial weather data sources and related metrics. We provide systematic evidence on measurement error introduced by 1) different methods used to obfuscate the exact GPS coordinates of households, 2) different metrics used to quantify precipitation and temperature, and 3) different remote sensing measurement technologies. First, we find no discernible effect of measurement error introduced by different obfuscation methods. Second, we find that simple weather metrics, such as total seasonal rainfall and mean daily temperature, outperform more complex metrics, such as deviations in rainfall from the long-run average or growing degree days, in a broad range of settings. Finally, we find substantial amounts of measurement error based on remote sensing product. In extreme cases, data drawn from different remote sensing products result in opposite signs for coefficients on weather metrics, meaning that precipitation or temperature draw from one product purportedly increases crop output while the same metrics drawn from a different product purportedly reduces crop output. We conclude with a set of six best practices for researchers looking to combine remote sensing weather data with socioeconomic survey data.

==> Estimating the Impact of Weather on Agriculture/tables/sumtab.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
\multicolumn{7}{l}{\emph{\textbf{Panel A}: Total Farm Production}}&            &            &            &            &            &            \\
Total farm production (2010 USD)&       245.4&       351.2&       188.5&       663.5&       207.3&       169.0\\
                    &     (322.8)&     (727.5)&     (201.7)&     (704.1)&     (269.4)&     (226.0)\\
Total farmed area (ha)&       1.055&       0.719&       11.14&       2.197&       1.598&       5.553\\
                    &     (5.670)&     (0.659)&     (15.59)&     (3.598)&     (2.985)&     (12.32)\\
Total farm yield (2010 USD/ha)&       440.6&       525.4&       60.93&       680.9&       235.2&       93.64\\
                    &     (607.2)&     (560.3)&     (169.0)&     (850.7)&     (286.8)&     (145.0)\\
Total farm labor rate (days/ha)&       434.4&       247.8&       94.94&       156.3&       311.1&       282.6\\
                    &     (834.9)&     (193.2)&     (219.1)&     (210.3)&     (353.9)&     (353.4)\\
Total farm fertilizer rate (kg/ha)&       56.26&       0.691&       5.120&       99.02&       20.89&       0.160\\
                    &     (94.98)&     (0.393)&     (23.83)&     (219.4)&     (68.17)&     (1.136)\\
Total farm pesticide use (\%)&      0.0615&      0.0418&      0.0800&       0.212&      0.0325&      0.0659\\
                    &     (0.240)&     (0.200)&     (0.271)&     (0.408)&     (0.177)&     (0.248)\\
Total farm herbicide use (\%)&       0.235&      0.0126&      0.0373&       0.292&      0.0981&      0.0295\\
                    &     (0.424)&     (0.112)&     (0.190)&     (0.455)&     (0.297)&     (0.169)\\
Total farm irrigation use (\%)&      0.0681&      0.0154&           0&      0.0270&      0.0422&      0.0202\\
                    &     (0.252)&     (0.123)&         (0)&     (0.162)&     (0.201)&     (0.141)\\
\midrule
\midrule Observations&        7272&        3250&        3913&        8384&        5669&        5250\\
\midrule
\multicolumn{7}{l}{\emph{\textbf{Panel B}: Primary Crop Production}}&            &            &            &            &            &            \\
Primary crop production (kg)&       314.6&       636.8&       471.5&       763.8&       608.5&       51.50\\
                    &     (476.6)&    (1035.3)&     (488.6)&    (1151.1)&     (793.5)&     (88.16)\\
Primary crop farmed area (ha)&       0.322&       0.661&       4.930&       0.720&       0.934&       1.501\\
                    &     (1.310)&     (0.622)&     (6.451)&     (1.115)&     (1.417)&     (2.669)\\
Primary crop yield (kg/ha)&      1593.2&      1191.8&       219.8&      1619.5&      1059.3&       87.89\\
                    &    (1782.8)&    (1242.1)&     (363.5)&    (2241.5)&    (1192.7)&     (146.7)\\
labor rate for maize (days/ha)&       466.1&       249.6&       70.72&       161.8&       263.2&       306.4\\
                    &     (666.6)&     (198.8)&     (121.1)&     (235.9)&     (295.9)&     (387.4)\\
Primary crop labor rate (days/ha)&       71.28&       0.722&       1.945&       146.3&       25.75&       0.196\\
                    &     (133.7)&     (0.399)&     (7.754)&     (302.0)&     (80.67)&     (1.638)\\
Primary crop pesticide use (\%)&      0.0259&      0.0388&      0.0550&       0.189&      0.0196&      0.0335\\
                    &     (0.159)&     (0.193)&     (0.228)&     (0.392)&     (0.139)&     (0.180)\\
Primary crop herbicide use (\%)&      0.0422&      0.0113&      0.0278&       0.378&      0.0945&      0.0219\\
                    &     (0.201)&     (0.106)&     (0.164)&     (0.485)&     (0.292)&     (0.146)\\
Primary crop irrigation use (\%)&      0.0515&      0.0141&           0&      0.0187&      0.0265&      0.0195\\
                    &     (0.221)&     (0.118)&         (0)&     (0.135)&     (0.161)&     (0.138)\\
\midrule
\midrule Observations&        3906&        3198&        3492&        3590&        4076&        2509\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_eth_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.58&        0.67&        0.67&        0.50&        0.83&        0.50\\
Median Daily Rainfall&        0.08&        0.83&        0.58&        0.25&        0.42&        0.50\\
Variance of Daily Rainfall&        0.58&        0.42&        0.58&        0.50&        0.67&        0.42\\
Skew of Daily Rainfall&        0.58&        0.50&        0.58&        0.75&        0.17&        0.25\\
Total Rainfall      &        0.58&        0.67&        0.67&        0.50&        0.83&        0.50\\
Deviation in Total Rainfall&        0.25&        0.58&        0.83&        0.00&        0.75&        0.17\\
Z-Score of Total Rainfall&        0.17&        0.42&        0.50&        0.17&        0.92&        0.25\\
Rainy Days          &        0.75&        0.67&        0.25&        0.83&        0.83&        0.92\\
Deviation in Rainy Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
No Rain Days        &        0.75&        0.33&        0.33&        0.83&        0.50&        0.75\\
Deviation in No Rain Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
\% Rainy Days       &        0.75&        0.67&        0.25&        0.83&        0.83&        0.92\\
Deviation in \% Rainy Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
Longest Dry Spell   &        0.33&        0.67&        0.42&        0.50&        0.42&        0.25\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_eth_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.67&        0.75&        0.50\\
Median Daily Temperature&        0.67&        0.58&        0.50\\
Variance of Daily Temperature&        0.33&        0.58&        0.50\\
Skew of Daily Temperature&        0.58&        0.25&        0.67\\
Growing Degree Days (GDD)&        0.17&        0.08&        0.33\\
Deviation in GDD    &        0.08&        0.25&        0.33\\
Z-Score of GDD      &        0.17&        0.25&        0.33\\
Maximum Daily Temperature&        0.33&        0.42&        0.42\\
\midrule
Observations        &          96&          96&          96\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_mwi_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.75&        0.67&        0.33&        0.67&        0.67&        0.75\\
Median Daily Rainfall&        0.17&        0.42&        0.92&        0.42&        0.50&        0.58\\
Variance of Daily Rainfall&        0.33&        0.33&        0.42&        0.17&        0.25&        0.33\\
Skew of Daily Rainfall&        0.92&        1.00&        0.42&        0.67&        0.08&        0.58\\
Total Rainfall      &        0.75&        0.67&        0.42&        0.67&        0.67&        0.75\\
Deviation in Total Rainfall&        0.17&        0.50&        0.33&        0.25&        0.67&        0.33\\
Z-Score of Total Rainfall&        0.25&        0.42&        0.33&        0.25&        0.33&        0.17\\
Rainy Days          &        0.67&        0.58&        0.42&        0.50&        0.42&        0.50\\
Deviation in Rainy Days&        0.75&        0.50&        0.67&        0.33&        0.58&        0.25\\
No Rain Days        &        0.67&        0.58&        0.42&        0.50&        0.50&        0.50\\
Deviation in No Rain Days&        0.75&        0.42&        0.67&        0.33&        0.58&        0.25\\
\% Rainy Days       &        0.67&        0.58&        0.42&        0.50&        0.42&        0.50\\
Deviation in \% Rainy Days&        0.75&        0.42&        0.67&        0.25&        0.58&        0.25\\
Longest Dry Spell   &        0.92&        0.58&        0.33&        0.58&        0.58&        0.25\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_mwi_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.92&        0.83&        0.67\\
Median Daily Temperature&        0.75&        0.83&        0.83\\
Variance of Daily Temperature&        0.50&        0.42&        0.58\\
Skew of Daily Temperature&        0.17&        0.25&        0.67\\
Growing Degree Days (GDD)&        0.83&        0.33&        0.42\\
Deviation in GDD    &        0.58&        0.42&        0.33\\
Z-Score of GDD      &        0.58&        0.58&        0.42\\
Maximum Daily Temperature&        0.58&        0.67&        0.67\\
\midrule
Observations        &          96&          96&          96\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_nga_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.58&        0.42&        0.58&        0.50&        0.83&        0.50\\
Median Daily Rainfall&        0.58&        0.33&        0.58&        0.58&        1.00&        0.58\\
Variance of Daily Rainfall&        0.75&        0.50&        0.25&        0.58&        0.83&        0.58\\
Skew of Daily Rainfall&        0.67&        0.42&        0.33&        0.42&        0.17&        0.42\\
Total Rainfall      &        0.58&        0.33&        0.67&        0.42&        0.83&        0.58\\
Deviation in Total Rainfall&        0.67&        0.50&        0.33&        0.50&        1.00&        0.50\\
Z-Score of Total Rainfall&        0.67&        0.92&        0.33&        0.17&        1.00&        0.67\\
Rainy Days          &        0.67&        0.50&        0.75&        0.67&        0.33&        0.75\\
Deviation in Rainy Days&        0.50&        0.58&        0.50&        0.58&        0.58&        0.58\\
No Rain Days        &        0.50&        0.42&        0.67&        0.42&        0.33&        0.58\\
Deviation in No Rain Days&        0.50&        0.58&        0.50&        0.58&        0.58&        0.58\\
\% Rainy Days       &        0.83&        0.58&        0.75&        0.83&        0.33&        0.92\\
Deviation in \% Rainy Days&        0.42&        0.75&        0.50&        0.33&        0.67&        0.58\\
Longest Dry Spell   &        0.42&        0.58&        0.33&        0.25&        0.58&        0.50\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_nga_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.58&        0.67&        0.58\\
Median Daily Temperature&        0.67&        0.75&        0.67\\
Variance of Daily Temperature&        0.75&        0.83&        0.58\\
Skew of Daily Temperature&        0.50&        0.42&        0.33\\
Growing Degree Days (GDD)&        0.75&        0.92&        0.83\\
Deviation in GDD    &        0.67&        0.67&        0.83\\
Z-Score of GDD      &        0.67&        0.83&        0.67\\
Maximum Daily Temperature&        0.67&        0.58&        0.58\\
\midrule
Observations        &          96&          96&          96\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_ngr_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.67&        0.67&        0.42&        0.67&        0.83&        0.33\\
Median Daily Rainfall&        0.00&        0.00&        0.58&        0.00&        0.00&        0.58\\
Variance of Daily Rainfall&        0.75&        0.83&        0.50&        0.67&        0.58&        0.25\\
Skew of Daily Rainfall&        0.42&        0.33&        0.42&        0.42&        0.42&        0.33\\
Total Rainfall      &        0.67&        0.67&        0.42&        0.67&        0.83&        0.33\\
Deviation in Total Rainfall&        0.58&        0.92&        0.83&        0.67&        0.67&        0.25\\
Z-Score of Total Rainfall&        0.58&        0.83&        0.83&        0.67&        0.50&        0.17\\
Rainy Days          &        0.42&        0.42&        0.58&        0.75&        0.67&        0.67\\
Deviation in Rainy Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
No Rain Days        &        0.50&        0.33&        0.58&        0.67&        0.58&        0.67\\
Deviation in No Rain Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
\% Rainy Days       &        0.42&        0.42&        0.58&        0.75&        0.67&        0.67\\
Deviation in \% Rainy Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
Longest Dry Spell   &        0.58&        0.75&        0.75&        0.42&        0.58&        0.75\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_ngr_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.50&        0.58&        0.58\\
Median Daily Temperature&        0.50&        0.67&        0.67\\
Variance of Daily Temperature&        0.50&        0.83&        0.50\\
Skew of Daily Temperature&        0.50&        0.50&        0.58\\
Growing Degree Days (GDD)&        0.50&        0.50&        0.75\\
Deviation in GDD    &        0.50&        0.50&        0.75\\
Z-Score of GDD      &        0.33&        0.67&        0.67\\
Maximum Daily Temperature&        0.83&        0.58&        0.83\\
\midrule
Observations        &          96&          96&          96\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_tza_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.33&        0.50&        0.50&        0.33&        0.42&        0.25\\
Median Daily Rainfall&        0.25&        0.08&        0.33&        0.25&        0.42&        0.25\\
Variance of Daily Rainfall&        0.25&        0.58&        0.58&        0.08&        0.25&        0.58\\
Skew of Daily Rainfall&        0.25&        0.50&        0.08&        0.42&        0.17&        0.25\\
Total Rainfall      &        0.33&        0.50&        0.50&        0.33&        0.42&        0.25\\
Deviation in Total Rainfall&        0.33&        0.33&        0.33&        0.17&        0.58&        0.17\\
Z-Score of Total Rainfall&        0.25&        0.50&        0.25&        0.17&        0.33&        0.17\\
Rainy Days          &        0.58&        0.58&        0.75&        0.50&        0.58&        0.42\\
Deviation in Rainy Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
No Rain Days        &        0.42&        0.75&        0.58&        0.50&        0.67&        0.33\\
Deviation in No Rain Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
\% Rainy Days       &        0.58&        0.58&        0.75&        0.50&        0.58&        0.42\\
Deviation in \% Rainy Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
Longest Dry Spell   &        0.08&        0.58&        0.17&        0.25&        0.25&        0.42\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_tza_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.50&        0.42&        0.33\\
Median Daily Temperature&        0.33&        0.58&        0.50\\
Variance of Daily Temperature&        0.67&        0.67&        0.58\\
Skew of Daily Temperature&        0.42&        0.33&        0.33\\
Growing Degree Days (GDD)&        0.00&        0.00&        0.67\\
Deviation in GDD    &        0.25&        0.00&        0.50\\
Z-Score of GDD      &        0.42&        0.00&        0.50\\
Maximum Daily Temperature&        0.33&        0.50&        0.42\\
\midrule
Observations        &          96&          96&          96\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_uga_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.33&        0.75&        0.58&        0.58&        0.58&        0.42\\
Median Daily Rainfall&        0.33&        0.08&        0.50&        0.33&        0.50&        0.50\\
Variance of Daily Rainfall&        0.42&        0.75&        0.67&        0.50&        0.67&        0.33\\
Skew of Daily Rainfall&        0.33&        0.42&        0.42&        0.17&        0.42&        0.50\\
Total Rainfall      &        0.33&        0.75&        0.67&        0.67&        0.58&        0.50\\
Deviation in Total Rainfall&        0.33&        0.58&        0.50&        0.58&        0.58&        0.58\\
Z-Score of Total Rainfall&        0.25&        0.42&        0.33&        0.58&        0.75&        0.58\\
Rainy Days          &        0.25&        0.58&        0.42&        0.50&        0.67&        0.67\\
Deviation in Rainy Days&        0.17&        0.33&        0.50&        0.58&        0.50&        0.67\\
No Rain Days        &        0.25&        0.58&        0.42&        0.42&        0.50&        0.67\\
Deviation in No Rain Days&        0.17&        0.42&        0.50&        0.58&        0.58&        0.67\\
\% Rainy Days       &        0.25&        0.58&        0.42&        0.42&        0.67&        0.67\\
Deviation in \% Rainy Days&        0.17&        0.33&        0.50&        0.58&        0.58&        0.67\\
Longest Dry Spell   &        0.50&        0.33&        0.50&        0.42&        0.58&        0.33\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sig_uga_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.58&        0.58&        0.42\\
Median Daily Temperature&        0.58&        0.58&        0.58\\
Variance of Daily Temperature&        0.42&        0.50&        0.17\\
Skew of Daily Temperature&        0.50&        0.50&        0.33\\
Growing Degree Days (GDD)&        0.25&        0.50&        0.50\\
Deviation in GDD    &        0.33&        0.67&        0.17\\
Z-Score of GDD      &        0.33&        0.33&        0.42\\
Maximum Daily Temperature&        0.50&        0.25&        0.67\\
\midrule
Observations        &          96&          96&          96\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sum_cp.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
Primary crop production (kg)&     314.628&     636.821&     471.515&     763.775&     608.486&      51.501\\
                    &   (476.561)&  (1035.265)&   (488.566)&  (1151.052)&   (793.543)&    (88.163)\\
Primary crop farmed area (ha)&       0.322&       0.661&       4.930&       0.720&       0.934&       1.501\\
                    &     (1.310)&     (0.622)&     (6.451)&     (1.115)&     (1.417)&     (2.669)\\
Primary crop yield (kg/ha)&    1593.185&    1191.798&     219.831&    1619.457&    1059.326&      87.887\\
                    &  (1782.828)&  (1242.061)&   (363.483)&  (2241.451)&  (1192.715)&   (146.689)\\
Primary crop labor rate (days/ha)&     466.074&     249.630&      70.716&     161.817&     263.232&     306.384\\
                    &   (666.579)&   (198.766)&   (121.063)&   (235.852)&   (295.932)&   (387.407)\\
Primary crop fertilizer rate (kg/ha)&      71.278&       0.722&       1.945&     146.287&      25.753&       0.196\\
                    &   (133.675)&     (0.399)&     (7.754)&   (302.022)&    (80.668)&     (1.638)\\
Primary crop pesticide use (\%)&       0.026&       0.039&       0.055&       0.189&       0.020&       0.033\\
                    &     (0.159)&     (0.193)&     (0.228)&     (0.392)&     (0.139)&     (0.180)\\
Primary crop herbicide use (\%)&       0.042&       0.011&       0.028&       0.378&       0.094&       0.022\\
                    &     (0.201)&     (0.106)&     (0.164)&     (0.485)&     (0.292)&     (0.146)\\
Primary crop irrigation use (\%)&       0.051&       0.014&       0.000&       0.019&       0.026&       0.020\\
                    &     (0.221)&     (0.118)&     (0.000)&     (0.135)&     (0.161)&     (0.138)\\
\midrule
Observations        &        3906&        3198&        3492&        3590&        4076&        2509\\


==> Estimating the Impact of Weather on Agriculture/tables/var_sum_tf.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
Total farm production (2010 USD)&     245.443&     351.200&     188.483&     663.534&     207.253&     168.963\\
                    &   (322.836)&   (727.512)&   (201.741)&   (704.067)&   (269.391)&   (226.006)\\
Total farmed area (ha)&       1.055&       0.719&      11.144&       2.197&       1.598&       5.553\\
                    &     (5.670)&     (0.659)&    (15.591)&     (3.598)&     (2.985)&    (12.319)\\
Total farm yield (2010 USD/ha)&     440.563&     525.363&      60.931&     680.936&     235.204&      93.638\\
                    &   (607.222)&   (560.263)&   (169.031)&   (850.662)&   (286.760)&   (145.023)\\
Total farm labor rate (days/ha)&     434.411&     247.781&      94.944&     156.287&     311.122&     282.568\\
                    &   (834.853)&   (193.168)&   (219.098)&   (210.296)&   (353.920)&   (353.363)\\
Total farm fertilizer rate (kg/ha)&      56.260&       0.691&       5.120&      99.021&      20.890&       0.160\\
                    &    (94.979)&     (0.393)&    (23.833)&   (219.442)&    (68.174)&     (1.136)\\
Total farm pesticide use (\%)&       0.061&       0.042&       0.080&       0.212&       0.032&       0.066\\
                    &     (0.240)&     (0.200)&     (0.271)&     (0.408)&     (0.177)&     (0.248)\\
Total farm herbicide use (\%)&       0.235&       0.013&       0.037&       0.292&       0.098&       0.030\\
                    &     (0.424)&     (0.112)&     (0.190)&     (0.455)&     (0.297)&     (0.169)\\
Total farm irrigation use (\%)&       0.068&       0.015&       0.000&       0.027&       0.042&       0.020\\
                    &     (0.252)&     (0.123)&     (0.000)&     (0.162)&     (0.201)&     (0.141)\\
\midrule
Observations        &        7272&        3250&        3913&        8384&        5669&        5250\\


==> tables/sumtab.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
\multicolumn{7}{l}{\emph{\textbf{Panel A}: Total Farm Production}}&            &            &            &            &            &            \\
Total farm production (2010 USD)&       245.4&       351.2&       188.5&       663.5&       207.3&       169.0\\
                    &     (322.8)&     (727.5)&     (201.7)&     (704.1)&     (269.4)&     (226.0)\\
Total farmed area (ha)&       1.055&       0.719&       11.14&       2.197&       1.598&       5.553\\
                    &     (5.670)&     (0.659)&     (15.59)&     (3.598)&     (2.985)&     (12.32)\\
Total farm yield (2010 USD/ha)&       440.6&       525.4&       60.93&       680.9&       235.2&       93.64\\
                    &     (607.2)&     (560.3)&     (169.0)&     (850.7)&     (286.8)&     (145.0)\\
Total farm labor rate (days/ha)&       434.4&       247.8&       94.94&       156.3&       311.1&       282.6\\
                    &     (834.9)&     (193.2)&     (219.1)&     (210.3)&     (353.9)&     (353.4)\\
Total farm fertilizer rate (kg/ha)&       56.26&       0.691&       5.120&       99.02&       20.89&       0.160\\
                    &     (94.98)&     (0.393)&     (23.83)&     (219.4)&     (68.17)&     (1.136)\\
Total farm pesticide use (\%)&      0.0615&      0.0418&      0.0800&       0.212&      0.0325&      0.0659\\
                    &     (0.240)&     (0.200)&     (0.271)&     (0.408)&     (0.177)&     (0.248)\\
Total farm herbicide use (\%)&       0.235&      0.0126&      0.0373&       0.292&      0.0981&      0.0295\\
                    &     (0.424)&     (0.112)&     (0.190)&     (0.455)&     (0.297)&     (0.169)\\
Total farm irrigation use (\%)&      0.0681&      0.0154&           0&      0.0270&      0.0422&      0.0202\\
                    &     (0.252)&     (0.123)&         (0)&     (0.162)&     (0.201)&     (0.141)\\
\midrule
\midrule Observations&        7272&        3250&        3913&        8384&        5669&        5250\\
\midrule
\multicolumn{7}{l}{\emph{\textbf{Panel B}: Primary Crop Production}}&            &            &            &            &            &            \\
Primary crop production (kg)&       314.6&       636.8&       471.5&       763.8&       608.5&       51.50\\
                    &     (476.6)&    (1035.3)&     (488.6)&    (1151.1)&     (793.5)&     (88.16)\\
Primary crop farmed area (ha)&       0.322&       0.661&       4.930&       0.720&       0.934&       1.501\\
                    &     (1.310)&     (0.622)&     (6.451)&     (1.115)&     (1.417)&     (2.669)\\
Primary crop yield (kg/ha)&      1593.2&      1191.8&       219.8&      1619.5&      1059.3&       87.89\\
                    &    (1782.8)&    (1242.1)&     (363.5)&    (2241.5)&    (1192.7)&     (146.7)\\
labor rate for maize (days/ha)&       466.1&       249.6&       70.72&       161.8&       263.2&       306.4\\
                    &     (666.6)&     (198.8)&     (121.1)&     (235.9)&     (295.9)&     (387.4)\\
Primary crop labor rate (days/ha)&       71.28&       0.722&       1.945&       146.3&       25.75&       0.196\\
                    &     (133.7)&     (0.399)&     (7.754)&     (302.0)&     (80.67)&     (1.638)\\
Primary crop pesticide use (\%)&      0.0259&      0.0388&      0.0550&       0.189&      0.0196&      0.0335\\
                    &     (0.159)&     (0.193)&     (0.228)&     (0.392)&     (0.139)&     (0.180)\\
Primary crop herbicide use (\%)&      0.0422&      0.0113&      0.0278&       0.378&      0.0945&      0.0219\\
                    &     (0.201)&     (0.106)&     (0.164)&     (0.485)&     (0.292)&     (0.146)\\
Primary crop irrigation use (\%)&      0.0515&      0.0141&           0&      0.0187&      0.0265&      0.0195\\
                    &     (0.221)&     (0.118)&         (0)&     (0.135)&     (0.161)&     (0.138)\\
\midrule
\midrule Observations&        3906&        3198&        3492&        3590&        4076&        2509\\


==> tables/var_sig_eth_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.58&        0.67&        0.67&        0.50&        0.83&        0.50\\
Median Daily Rainfall&        0.08&        0.83&        0.58&        0.25&        0.42&        0.50\\
Variance of Daily Rainfall&        0.58&        0.42&        0.58&        0.50&        0.67&        0.42\\
Skew of Daily Rainfall&        0.58&        0.50&        0.58&        0.75&        0.17&        0.25\\
Total Rainfall      &        0.58&        0.67&        0.67&        0.50&        0.83&        0.50\\
Deviation in Total Rainfall&        0.25&        0.58&        0.83&        0.00&        0.75&        0.17\\
Z-Score of Total Rainfall&        0.17&        0.42&        0.50&        0.17&        0.92&        0.25\\
Rainy Days          &        0.75&        0.67&        0.25&        0.83&        0.83&        0.92\\
Deviation in Rainy Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
No Rain Days        &        0.75&        0.33&        0.33&        0.83&        0.50&        0.75\\
Deviation in No Rain Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
\% Rainy Days       &        0.75&        0.67&        0.25&        0.83&        0.83&        0.92\\
Deviation in \% Rainy Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
Longest Dry Spell   &        0.33&        0.67&        0.42&        0.50&        0.42&        0.25\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_eth_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.67&        0.75&        0.50\\
Median Daily Temperature&        0.67&        0.58&        0.50\\
Variance of Daily Temperature&        0.33&        0.58&        0.50\\
Skew of Daily Temperature&        0.58&        0.25&        0.67\\
Growing Degree Days (GDD)&        0.17&        0.08&        0.33\\
Deviation in GDD    &        0.08&        0.25&        0.33\\
Z-Score of GDD      &        0.17&        0.25&        0.33\\
Maximum Daily Temperature&        0.33&        0.42&        0.42\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_mwi_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.75&        0.67&        0.33&        0.67&        0.67&        0.75\\
Median Daily Rainfall&        0.17&        0.42&        0.92&        0.42&        0.50&        0.58\\
Variance of Daily Rainfall&        0.33&        0.33&        0.42&        0.17&        0.25&        0.33\\
Skew of Daily Rainfall&        0.92&        1.00&        0.42&        0.67&        0.08&        0.58\\
Total Rainfall      &        0.75&        0.67&        0.42&        0.67&        0.67&        0.75\\
Deviation in Total Rainfall&        0.17&        0.50&        0.33&        0.25&        0.67&        0.33\\
Z-Score of Total Rainfall&        0.25&        0.42&        0.33&        0.25&        0.33&        0.17\\
Rainy Days          &        0.67&        0.58&        0.42&        0.50&        0.42&        0.50\\
Deviation in Rainy Days&        0.75&        0.50&        0.67&        0.33&        0.58&        0.25\\
No Rain Days        &        0.67&        0.58&        0.42&        0.50&        0.50&        0.50\\
Deviation in No Rain Days&        0.75&        0.42&        0.67&        0.33&        0.58&        0.25\\
\% Rainy Days       &        0.67&        0.58&        0.42&        0.50&        0.42&        0.50\\
Deviation in \% Rainy Days&        0.75&        0.42&        0.67&        0.25&        0.58&        0.25\\
Longest Dry Spell   &        0.92&        0.58&        0.33&        0.58&        0.58&        0.25\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_mwi_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.92&        0.83&        0.67\\
Median Daily Temperature&        0.75&        0.83&        0.83\\
Variance of Daily Temperature&        0.50&        0.42&        0.58\\
Skew of Daily Temperature&        0.17&        0.25&        0.67\\
Growing Degree Days (GDD)&        0.83&        0.33&        0.42\\
Deviation in GDD    &        0.58&        0.42&        0.33\\
Z-Score of GDD      &        0.58&        0.58&        0.42\\
Maximum Daily Temperature&        0.58&        0.67&        0.67\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_nga_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.58&        0.42&        0.58&        0.50&        0.83&        0.50\\
Median Daily Rainfall&        0.58&        0.33&        0.58&        0.58&        1.00&        0.58\\
Variance of Daily Rainfall&        0.75&        0.50&        0.25&        0.58&        0.83&        0.58\\
Skew of Daily Rainfall&        0.67&        0.42&        0.33&        0.42&        0.17&        0.42\\
Total Rainfall      &        0.58&        0.33&        0.67&        0.42&        0.83&        0.58\\
Deviation in Total Rainfall&        0.67&        0.50&        0.33&        0.50&        1.00&        0.50\\
Z-Score of Total Rainfall&        0.67&        0.92&        0.33&        0.17&        1.00&        0.67\\
Rainy Days          &        0.67&        0.50&        0.75&        0.67&        0.33&        0.75\\
Deviation in Rainy Days&        0.50&        0.58&        0.50&        0.58&        0.58&        0.58\\
No Rain Days        &        0.50&        0.42&        0.67&        0.42&        0.33&        0.58\\
Deviation in No Rain Days&        0.50&        0.58&        0.50&        0.58&        0.58&        0.58\\
\% Rainy Days       &        0.83&        0.58&        0.75&        0.83&        0.33&        0.92\\
Deviation in \% Rainy Days&        0.42&        0.75&        0.50&        0.33&        0.67&        0.58\\
Longest Dry Spell   &        0.42&        0.58&        0.33&        0.25&        0.58&        0.50\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_nga_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.58&        0.67&        0.58\\
Median Daily Temperature&        0.67&        0.75&        0.67\\
Variance of Daily Temperature&        0.75&        0.83&        0.58\\
Skew of Daily Temperature&        0.50&        0.42&        0.33\\
Growing Degree Days (GDD)&        0.75&        0.92&        0.83\\
Deviation in GDD    &        0.67&        0.67&        0.83\\
Z-Score of GDD      &        0.67&        0.83&        0.67\\
Maximum Daily Temperature&        0.67&        0.58&        0.58\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_ngr_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.67&        0.67&        0.42&        0.67&        0.83&        0.33\\
Median Daily Rainfall&        0.00&        0.00&        0.58&        0.00&        0.00&        0.58\\
Variance of Daily Rainfall&        0.75&        0.83&        0.50&        0.67&        0.58&        0.25\\
Skew of Daily Rainfall&        0.42&        0.33&        0.42&        0.42&        0.42&        0.33\\
Total Rainfall      &        0.67&        0.67&        0.42&        0.67&        0.83&        0.33\\
Deviation in Total Rainfall&        0.58&        0.92&        0.83&        0.67&        0.67&        0.25\\
Z-Score of Total Rainfall&        0.58&        0.83&        0.83&        0.67&        0.50&        0.17\\
Rainy Days          &        0.42&        0.42&        0.58&        0.75&        0.67&        0.67\\
Deviation in Rainy Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
No Rain Days        &        0.50&        0.33&        0.58&        0.67&        0.58&        0.67\\
Deviation in No Rain Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
\% Rainy Days       &        0.42&        0.42&        0.58&        0.75&        0.67&        0.67\\
Deviation in \% Rainy Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
Longest Dry Spell   &        0.58&        0.75&        0.75&        0.42&        0.58&        0.75\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_ngr_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.50&        0.58&        0.58\\
Median Daily Temperature&        0.50&        0.67&        0.67\\
Variance of Daily Temperature&        0.50&        0.83&        0.50\\
Skew of Daily Temperature&        0.50&        0.50&        0.58\\
Growing Degree Days (GDD)&        0.50&        0.50&        0.75\\
Deviation in GDD    &        0.50&        0.50&        0.75\\
Z-Score of GDD      &        0.33&        0.67&        0.67\\
Maximum Daily Temperature&        0.83&        0.58&        0.83\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_tza_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.33&        0.50&        0.50&        0.33&        0.42&        0.25\\
Median Daily Rainfall&        0.25&        0.08&        0.33&        0.25&        0.42&        0.25\\
Variance of Daily Rainfall&        0.25&        0.58&        0.58&        0.08&        0.25&        0.58\\
Skew of Daily Rainfall&        0.25&        0.50&        0.08&        0.42&        0.17&        0.25\\
Total Rainfall      &        0.33&        0.50&        0.50&        0.33&        0.42&        0.25\\
Deviation in Total Rainfall&        0.33&        0.33&        0.33&        0.17&        0.58&        0.17\\
Z-Score of Total Rainfall&        0.25&        0.50&        0.25&        0.17&        0.33&        0.17\\
Rainy Days          &        0.58&        0.58&        0.75&        0.50&        0.58&        0.42\\
Deviation in Rainy Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
No Rain Days        &        0.42&        0.75&        0.58&        0.50&        0.67&        0.33\\
Deviation in No Rain Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
\% Rainy Days       &        0.58&        0.58&        0.75&        0.50&        0.58&        0.42\\
Deviation in \% Rainy Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
Longest Dry Spell   &        0.08&        0.58&        0.17&        0.25&        0.25&        0.42\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_tza_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.50&        0.42&        0.33\\
Median Daily Temperature&        0.33&        0.58&        0.50\\
Variance of Daily Temperature&        0.67&        0.67&        0.58\\
Skew of Daily Temperature&        0.42&        0.33&        0.33\\
Growing Degree Days (GDD)&        0.00&        0.00&        0.67\\
Deviation in GDD    &        0.25&        0.00&        0.50\\
Z-Score of GDD      &        0.42&        0.00&        0.50\\
Maximum Daily Temperature&        0.33&        0.50&        0.42\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_uga_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.33&        0.75&        0.58&        0.58&        0.58&        0.42\\
Median Daily Rainfall&        0.33&        0.08&        0.50&        0.33&        0.50&        0.50\\
Variance of Daily Rainfall&        0.42&        0.75&        0.67&        0.50&        0.67&        0.33\\
Skew of Daily Rainfall&        0.33&        0.42&        0.42&        0.17&        0.42&        0.50\\
Total Rainfall      &        0.33&        0.75&        0.67&        0.67&        0.58&        0.50\\
Deviation in Total Rainfall&        0.33&        0.58&        0.50&        0.58&        0.58&        0.58\\
Z-Score of Total Rainfall&        0.25&        0.42&        0.33&        0.58&        0.75&        0.58\\
Rainy Days          &        0.25&        0.58&        0.42&        0.50&        0.67&        0.67\\
Deviation in Rainy Days&        0.17&        0.33&        0.50&        0.58&        0.50&        0.67\\
No Rain Days        &        0.25&        0.58&        0.42&        0.42&        0.50&        0.67\\
Deviation in No Rain Days&        0.17&        0.42&        0.50&        0.58&        0.58&        0.67\\
\% Rainy Days       &        0.25&        0.58&        0.42&        0.42&        0.67&        0.67\\
Deviation in \% Rainy Days&        0.17&        0.33&        0.50&        0.58&        0.58&        0.67\\
Longest Dry Spell   &        0.50&        0.33&        0.50&        0.42&        0.58&        0.33\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_uga_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.58&        0.58&        0.42\\
Median Daily Temperature&        0.58&        0.58&        0.58\\
Variance of Daily Temperature&        0.42&        0.50&        0.17\\
Skew of Daily Temperature&        0.50&        0.50&        0.33\\
Growing Degree Days (GDD)&        0.25&        0.50&        0.50\\
Deviation in GDD    &        0.33&        0.67&        0.17\\
Z-Score of GDD      &        0.33&        0.33&        0.42\\
Maximum Daily Temperature&        0.50&        0.25&        0.67\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sum_cp.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
Primary crop production (kg)&     314.628&     636.821&     471.515&     763.775&     608.486&      51.501\\
                    &   (476.561)&  (1035.265)&   (488.566)&  (1151.052)&   (793.543)&    (88.163)\\
Primary crop farmed area (ha)&       0.322&       0.661&       4.930&       0.720&       0.934&       1.501\\
                    &     (1.310)&     (0.622)&     (6.451)&     (1.115)&     (1.417)&     (2.669)\\
Primary crop yield (kg/ha)&    1593.185&    1191.798&     219.831&    1619.457&    1059.326&      87.887\\
                    &  (1782.828)&  (1242.061)&   (363.483)&  (2241.451)&  (1192.715)&   (146.689)\\
Primary crop labor rate (days/ha)&     466.074&     249.630&      70.716&     161.817&     263.232&     306.384\\
                    &   (666.579)&   (198.766)&   (121.063)&   (235.852)&   (295.932)&   (387.407)\\
Primary crop fertilizer rate (kg/ha)&      71.278&       0.722&       1.945&     146.287&      25.753&       0.196\\
                    &   (133.675)&     (0.399)&     (7.754)&   (302.022)&    (80.668)&     (1.638)\\
Primary crop pesticide use (\%)&       0.026&       0.039&       0.055&       0.189&       0.020&       0.033\\
                    &     (0.159)&     (0.193)&     (0.228)&     (0.392)&     (0.139)&     (0.180)\\
Primary crop herbicide use (\%)&       0.042&       0.011&       0.028&       0.378&       0.094&       0.022\\
                    &     (0.201)&     (0.106)&     (0.164)&     (0.485)&     (0.292)&     (0.146)\\
Primary crop irrigation use (\%)&       0.051&       0.014&       0.000&       0.019&       0.026&       0.020\\
                    &     (0.221)&     (0.118)&     (0.000)&     (0.135)&     (0.161)&     (0.138)\\
\midrule
Observations        &        3906&        3198&        3492&        3590&        4076&        2509\\


==> tables/var_sum_tf.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
Total farm production (2010 USD)&     245.443&     351.200&     188.483&     663.534&     207.253&     168.963\\
                    &   (322.836)&   (727.512)&   (201.741)&   (704.067)&   (269.391)&   (226.006)\\
Total farmed area (ha)&       1.055&       0.719&      11.144&       2.197&       1.598&       5.553\\
                    &     (5.670)&     (0.659)&    (15.591)&     (3.598)&     (2.985)&    (12.319)\\
Total farm yield (2010 USD/ha)&     440.563&     525.363&      60.931&     680.936&     235.204&      93.638\\
                    &   (607.222)&   (560.263)&   (169.031)&   (850.662)&   (286.760)&   (145.023)\\
Total farm labor rate (days/ha)&     434.411&     247.781&      94.944&     156.287&     311.122&     282.568\\
                    &   (834.853)&   (193.168)&   (219.098)&   (210.296)&   (353.920)&   (353.363)\\
Total farm fertilizer rate (kg/ha)&      56.260&       0.691&       5.120&      99.021&      20.890&       0.160\\
                    &    (94.979)&     (0.393)&    (23.833)&   (219.442)&    (68.174)&     (1.136)\\
Total farm pesticide use (\%)&       0.061&       0.042&       0.080&       0.212&       0.032&       0.066\\
                    &     (0.240)&     (0.200)&     (0.271)&     (0.408)&     (0.177)&     (0.248)\\
Total farm herbicide use (\%)&       0.235&       0.013&       0.037&       0.292&       0.098&       0.030\\
                    &     (0.424)&     (0.112)&     (0.190)&     (0.455)&     (0.297)&     (0.169)\\
Total farm irrigation use (\%)&       0.068&       0.015&       0.000&       0.027&       0.042&       0.020\\
                    &     (0.252)&     (0.123)&     (0.000)&     (0.162)&     (0.201)&     (0.141)\\
\midrule
Observations        &        7272&        3250&        3913&        8384&        5669&        5250\\

